Provably Efficient Q-Learning with Low Switching Cost

We take initial steps in studying PAC-MDP algorithms with limited adaptivity, that is, algorithms that change its exploration policy as infrequently as possible during regret minimization. This is motivated by the difficulty of running fully adaptive algorithms in real-world applications (such as medical domains), and we propose to quantify adaptivity using the notion of local switching cost. Our main contribution, Q-Learning with UCB2 exploration, is a model-free algorithm for H-step episodic MDP that achieves sublinear regret whose local switching cost in K episodes is $O(H^3SA\log K)$, and we provide a lower bound of $\Omega(HSA)$ on the local switching cost for any no-regret algorithm. Our algorithm can be naturally adapted to the concurrent setting, which yields nontrivial results that improve upon prior work in certain aspects.

==> Sections/todo.tex <==
\section*{TODOs}
\begin{enumerate}
\item Writing:
  \begin{enumerate}[a.]
  \item Rewrite the intro.
  \item Write the prior work section.
  \item Go through sections 2 - 4 and polish the writing.
  \item Revise the abstract.
  \end{enumerate}
\item Lower bound on switching cost (Section 7).
  \begin{enumerate}[a.]
  \item Rigorize and write the $\Omega(HSA)$ lower bound.
  \item Discussions on $\log\log T$ and factor in $H$.
  \end{enumerate}
\item Notation:
  % \begin{enumerate}[a.]
  % \item Change $\alpha$ to something else (e.g. $\eta$). Should be a
  %   one time thing.
  % \end{enumerate}
% \item Algorithms with better \emph{global switching cost}?
%   \yub{Defined, but probably skipping further discussions.}
%   \yub{Reviewers could highly likely ask this.}
% \item Justification and application of low switching cost:
%   \begin{enumerate}[a.]
%   \item DONE. Connection to concurrent RL.
%   \item Other justifications? e.g. Cesa-Bianchi 2013?
%   \end{enumerate}
% \item DONE. Adapt UCB2 to better regret bound algorithms: Bernstein
%   Q-Learning
  % \yub{Tengyang's working on this}.
  % {Hoeffding, Bernstein} model-based RL
  % of~\cite{azar2017minimax}~\yub{not sure due to the issue in their
  %   proof.}
\end{enumerate}
